DinoSR: Self-Distillation and Online Clustering for Self-supervised Speech Representation Learning

In this paper, we introduce self-distillation and online clustering for self-supervised speech representation learning (DinoSR) which combines masked language modeling, self-distillation, and online clustering. We show that these concepts complement each other and result in a strong representation learning model for speech. DinoSR first extracts contextualized embeddings from the input audio with a teacher network, then runs an online clustering system on the embeddings to yield a machine-discovered phone inventory, and finally uses the discretized tokens to guide a student network. We show that DinoSR surpasses previous state-of-the-art performance in several downstream tasks, and provide a detailed analysis of the model and the learned discrete units.

==> figures/mask.tex <==
\begin{figure}[!h]
% \vspace{-10pt}
\begin{center}
\centerline{\includegraphics[width=0.4\linewidth]{mask.pdf}}
\end{center}
% \vspace{-30pt}
\caption{Varying the input masked ratio $M$ of the student network.}
\label{fig:mask}
\vspace{-10pt}
\end{figure}


